Membership Privacy for Machine Learning Models Through Knowledge Transfer

Large capacity machine learning (ML) models are prone to membership inference attacks (MIAs), which aim to infer whether the target sample is a member of the target model's training dataset. The serious privacy concerns due to the membership inference have motivated multiple defenses against MIAs, e.g., differential privacy and adversarial regularization. Unfortunately, these defenses produce ML models with unacceptably low classification performances. Our work proposes a new defense, called distillation for membership privacy (DMP), against MIAs that preserves the utility of the resulting models significantly better than prior defenses. DMP leverages knowledge distillation to train ML models with membership privacy. We provide a novel criterion to tune the data used for knowledge transfer in order to amplify the membership privacy of DMP. Our extensive evaluation shows that DMP provides significantly better tradeoffs between membership privacy and classification accuracies compared to state-of-the-art MIA defenses. For instance, DMP achieves ~100% accuracy improvement over adversarial regularization for DenseNet trained on CIFAR100, for similar membership privacy (measured using MIA risk): when the MIA risk is 53.7%, adversarially regularized DenseNet is 33.6% accurate, while DMP-trained DenseNet is 65.3% accurate.

==> adaptive_adv.tex <==
% !TEX root = main.tex

% \vspace{-3em}
\subsection{Discussions}\label{adaptive}


\subsubsection{Why does DMP work better?}\label{why}
As discussed in~\cite{long2018understanding}, membership inference attacks exploit the \emph{unique influence} of a member record on the target model. 
To prevent this, DMP trains an unprotected model, $\theta_\mathsf{up}$, on private training data, $D_\mathsf{tr}$, and  uses predictions of $\theta_\mathsf{up}$ on a reference data, $X_\mathsf{ref}$, to train its final protected model, $\theta_\mathsf{p}$.
Therefore, DMP reduces the influence of $D_\mathsf{tr}$ by hindering the direct access of $\theta_\mathsf{p}$ to $D_\mathsf{tr}$. We also show membership privacy can be further strengthened by selecting $X_\mathsf{ref}$ with low entropy predictions.
Note that low entropy $X_\mathsf{ref}$ are ``easy-to-classify'' samples whose predictions are  not affected by small changes in $D_\mathsf{tr}$. Therefore, $\theta_\mathsf{p}$ trained on these predictions preserves membership privacy of $D_\mathsf{tr}$.



The main goal of DMP is to improve privacy-utility tradeoffs of ML models, i.e., increase the prediction accuracy of a model for a given level of membership privacy.
Both regularization and differential privacy mechanisms can achieve any level of membership privacy. But, with the same membership privacy, DMP models have significantly better prediction accuracies than conventionally regularized or DP models.
This is because \emph{DMP incorporates utility in its objective}: More specifically, it forces the predictions of $\theta_\mathsf{p}$ and $\theta_\mathsf{up}$ on non-member data, $X_\mathsf{ref}$, to be the same, using  soft labels based loss function in~\eqref{kld_datum}, and effectively transfers the prediction accuracy of $\theta_\mathsf{up}$ to $\theta_\mathsf{p}$. 
On the contrary, DP mechanisms~\cite{abadi2016deep,papernot2017semi} add noise calibrated to satisfy DP guarantees and do not incorporate utility constraints, which makes training highly accurate DP models challenging.




On the other hand, the loss of adversarial regularization puts different weights on two terms: first, the classification loss computed by directly accessing $D_\mathsf{tr}$, and second, the accuracy of the membership inference attack to be mitigated. Due to the direct access to $D_\mathsf{tr}$, to reduce overfitting, the weight on the second term needs to be high as proposed in the original work~\cite{nasr2018machine}. The goal of the second term is to train the final model to fool the attack model, and therefore, it does not help to improve the prediction accuracy of the final model. Therefore, the higher weight on the second term significantly harms the accuracy of the final model.
In self-distillation~\cite{hinton2014distilling,papernot2016distillation}, soft predictions of a model on its own training data are used to improve generalization of the model without compromising the model accuracy.
DMP uses predictions on reference data, disjoint from the private training data, to train its final model. This achieves high prediction accuracy due to the high quality predictions, while providing strong membership privacy.




\subsubsection{Synthetic reference data for DMP}\label{adaptive:synth}
An important requirement of DMP is access to some reference data for distillation. 
First, as mentioned before, DMP uses \emph{unlabeled} reference data; 
most data owners have access to huge amounts of unlabeled data, but labeled data is scarce due to the expensive process of manual labeling. In our setting, the data owners will not even release their unlabeled reference data that may be sensitive.   
Second, even if a DMP trainer does not have access to enough unlabeled reference data, she can generate \emph{synthetic} (unlabeled) reference data through different means such as generative adversarial networks.
Specifically, we synthesized reference data for CIFAR-10 using the DC-GAN architecture \cite{radford2015unsupervised}.
With 25,000 of \textbf{real} CIFAR-10 data as its reference data, DMP achieves a ($E_\mathsf{gen}$, $A_\mathsf{te}$, $A_\mathsf{bb}$) of (3.1, 65.0, 50.6) (Table \ref{table:performance_comparison}).
On the other hand, by using 
 25,000 of \textbf{synthetic} CIFAR-10 data generated using DC-GAN, DMP achieves a ($E_\mathsf{gen}$, $A_\mathsf{te}$, $A_\mathsf{bb}$) of (3.5, 56.8, 51.3); these results are close to when non-synthetic CIFAR-10 reference data is used.
As the distribution of synthetic reference data does not exactly match that of real data, the corresponding DMP models have slightly poorer generalization and test accuracies; this can be improved with better generative models.
The larger the synthetic reference data, the better the final DMP models: For 12500, 25000, and 37500 amounts of synthetic reference data, we obtain a ($E_\mathsf{gen}$, $A_\mathsf{te}$, $A_\mathsf{bb}$) of (2.1, 53.0, 50.3), (3.5, 56.8, 51.3), and (5.0, 57.5, 52.1), respectively.
This shows that DMP does not necessarily need real reference data and, and it still outperforms existing defenses even with  synthetic reference data.
Recent work has also  investigated generating categorical data~\cite{gal2015latent,camino2018generating} using more classical methods.e


\subsubsection{Adaptive attacks on DMP}\label{adaptive:attack}
%
An adversary may try to adapt her attack against DMP, by leveraging DMP's particular reference data selection, which is based on the entropy  of predictions of $\theta_\mathsf{up}$. 
However, as discussed in our threat model (Section \ref{prelim:threat}), we assume the reference data is \textbf{not publicly available} due to its possibly sensitive nature.
Hence, the adversary first needs to identify the reference data, e.g., by mounting a membership inference attack on $\theta_\mathsf{p}$; 
% 
however, as shown in Section~\ref{exp:ref_risk}, such an attack is highly infeasible since our reference data samples do not have hard labels (but soft labels distilled from the original training data). 
Hence, the adversary cannot obtain the reference dataset to adapt her attack.




Next, we show that even if the adversary can obtain the  reference data accurately, e.g., through out of band channels, adaptive attacks cannot be effective.
In DMP, reference samples have low entropy predictions of $\theta_\mathsf{up}$, but members of training data of $\theta_\mathsf{up}$ also have low entropies, due to overfitting.
Therefore, training data members and low entropy reference samples could be similar, i.e., close in feature space.
%
The adversary can exploit this possibility by measuring distances of given target sample to the reference data and inferring that the target sample is a member if it is close to the reference data with low entropy predictions.
However, we show that the proximity of samples in feature space does not correlate with the closeness of their entropy, i.e., a low distance between a target sample and reference samples with low entropy does not imply that the target sample also has low entropy or is a member, and vice-versa.
In other words, \emph{closeness of samples in the feature space cannot be exploited to strengthen membership inference.}


Figure~\ref{fig:aa_dist} demonstrates this for Purchase-100 dataset; this dataset has binary features, therefore, we use the hamming distance.
Each point refers to a target member or non-member sample, and reference samples on x-axis are arranged in increasing order of entropy from left to right.
The X-axis shows the reference sample closest to a given target sample and the Y-axis shows the distance between these two samples in the feature space.
As members and non-members are not separated along either of the axes, there is no correlation between the closeness in feature space and the closeness of entropies.
Hence, adaptive attacks exploiting distances between samples in feature space will not gain any membership information.





\begin{figure}[h]

\centering
\includegraphics[scale=0.32]{./figures/adaptive_dist_based.pdf}
\caption{Closeness of reference and target samples in feature space does not correlate with closeness of entropy, which makes distance based adaptive attack against DMP impossible. Experiment performed for Purchase-100 dataset.}
\label{fig:aa_dist}
\end{figure}


==> related1.tex <==
% !TEX root = main.tex
\section{Related Work}\label{related_work}





Privacy preserving machine learning is an active area of research.
Multiple inference attacks against ML models are proposed in literature, e.g., input inference~\cite{fredrikson2015model}, blackbox and whitebox membership inference~\cite{shokri2017membership,nasr2019comprehensive,salem2018ml,leino2019stolen}, attribute inference~\cite{carlini2018secret}, parameter inference~\cite{tramer2016stealing,wang2018stealing}, training data embedding attacks~\cite{song2017machine}, and side-channel attacks~\cite{wei2018know}.
In this paper, we focus on the membership inference attacks for adversaries with  blackbox and whitebox access to the model.








Several defenses have been proposed against  membership inference attacks~\cite{abadi2016deep,papernot2018scalable,nasr2018machine,papernot2017semi}.
Unfortunately, the existing defenses do not provide acceptable tradeoffs between privacy and utility, i.e., they  hurt the model's classification performance significantly to provide membership privacy.  
Defenses based on differential privacy (DP) \cite{abadi2016deep,papernot2018scalable,papernot2017semi,hamm2016learning,pathak2010multiparty} provide rigorous membership privacy guarantees, but as demonstrated by Jayaraman et al. \cite{jayaraman2019evaluating}, the resulting models are of no practical use.
Furthremore, as \cite{jayaraman2019evaluating,leino2019stolen} shows---and we confirm in our work---with relaxed privacy budgets, DP defenses are also susceptible to the membership inference.
The primary reason for the susceptibility is the high generalization error of such models, which is sufficient for membership inference~\cite{long2018understanding,rahman2018membership,shokri2017membership,nasr2019comprehensive,leino2019stolen}.
Adversarial regularization~\cite{nasr2018machine} is a recent defense that is tailored to  membership inference attacks, and claims to improve the tradeoffs.
However, as shown in Section~\ref{exp:regularizations}, the adversarial regularization defense fails to provide acceptable tradeoffs when evaluated against state-of-the-art membership inference attacks.







Knowledge distillation has been used in 
several privacy defenses \cite{papernot2017semi,hamm2016learning,pathak2010multiparty,nissim2007smooth,bassily2018model,wang2019private}, which perform distillation using a noisy aggregate of predictions of models of multiple data holders.
In particular, PATE~\cite{papernot2017semi,papernot2018scalable} combines knowledge distillation and DP~\cite{abadi2016deep}.
In PATE, an input is labeled by an ensemble of \emph{teacher models}, and the final \emph{student model} is trained using the noisy aggregates of all  labels.
We perform a comprehensive comparison of DMP and PATE in Section \ref{exp:dp} to show that DMP provides better tradeoffs between membership privacy and accuracy.
% PATE requires exorbitantly large amounts of data to train a good teachers' ensemble, whose knowledge is transferred to the student model
% In the absence of such data, the aggregation in PATE does not produce sufficient number of labels at low privacy budgets, and therefore, cannot train accurate student models; we demonstrate this in Section \ref{exp:dp}.
% Even at higher privacy budgets, PATE-trained students do not attain the accuracy similar to DMP-trained models, because, the ensemble used to transfer knowledge in PATE is significantly less accurate than the unprotected model used in DMP.
% In effect, DMP provides better tradeoffs than PATE.
DP defenses add large amounts of noise to provide privacy to \emph{any data} with the underlying distribution, and in this process incur high accuracy losses~\cite{papernot2018scalable}.
However, due to the targeted motivation to provide membership privacy, instead of adding any explicit noise, DMP defense uses the novel knowledge transfer via easy-to-classify samples, whose predictions are not affected by the presence of any particular member in the private training data.
% Therefore, our approach differs from these defenses in that, we do not explicitly add DP noise, and instead, prevent the membership leakage through the predictions of the reference data.





Regularization alone is shown to be ineffective against membership inference attacks \cite{long2018understanding,nasr2019comprehensive,leino2019stolen}.
Long et al. \cite{long2018understanding} proposed a  membership inference attack against well-generalized models that identifies the vulnerable \emph{outliers} in the sensitive training data of the model, whose membership can be inferred.
In DMP, such outliers can be protected by setting high softmax temperatures or selecting samples with low entropy predictions (Section \ref{dmp:analysis}), but at the cost of utility degradation.
This is similar to  previous defenses: in DP-SGD, privacy budget is reduced and in the adversarial regularization, high regularization factor is set to provide privacy to the outliers, and in practice, at relaxed privacy budgets or low regularization factors, these defenses also pose the membership inference risk to such outliers \cite{jayaraman2019evaluating,rahman2018membership}.
% Leino et al. \cite{leino2019stolen} also proposed whitebox membership inference attacks against well-generalized models, including differentially private models.
However, we note that the primary objective of our DMP  defense is to produce models with superior tradeoffs, i.e., achieve superior classification performance for a given degree of membership privacy.
We demonstrated the effectiveness of DMP in Section \ref{exp} in producing such models with state-of-the-art classification accuracy for a given membership privacy.









% To summarize, \emph{all of the existing defenses rely on adding some explicit noise during the training or regularization of the model} in different ways.
% Because of such  explicit noise additions, all these defenses suffer from  significant utility degradations in terms of classification performance of the final models.
% By contrast, DMP provides membership inference resistance using a novel approach of selecting low entropy easy-to-classify samples for knowledge transfer.
% Knowledge transfer presents itself as a promising option for practical utility-membership privacy tradeoffs  because of its proven ability to transfer the utility of the cumbersome model to the final model~\cite{hinton2014distilling,wang2019private,ba2014deep}.


